Unified Low Complexity Radix-2 Architectures for Time and Frequency-domain GFDM Modem

Most of the conventional multicarrier waveforms explicitly or implicitly involve a generalized frequency division multiplexing (GFDM)-based modem as a core part of the baseband processing. Some are based on GFDM with a single prototype filter, e.g. orthogonal frequency division multiplexing (OFDM) and others employ multiple filters such as filter bank multicarrier (FBMC). Moreover, the GFDM degrees of freedom combined with multiple prototype filters design allow the development and optimization of new waveforms. Nevertheless, GFDM has been widely considered as a complex modulation because of the requirements of odd number of subcarriers or subsymbols. Accordingly, the current state of the art implementations consume high resources. One solution to reduce the complexity is utilizing radix-2 parameters. Due to the advancement in GFDM filter design, the constraint of using odd parameters has been overcome and radix-2 realization is now possible. In this paper, we propose a unified low complexity architecture that can be reconfigured to provide both time-domain and frequency-domain modulation/demodulation. The design consists of several radix-2 fast Fourier transform (FFT) and memory blocks, in addition to one complex multiplier. Moreover, we provide a unified architecture for the state of the art implementations, which is designed based on direct computation of circular convolution using parallel multiplier chains. As we demonstrate in this work, the FFTbased architecture is computationally more efficient, provides more flexibility, significantly reduces the resource consumption, and achieves similar latency for larger block size.

==> 7_acknowledgment.tex <==
\section*{Acknowledgment}
The work presented in this paper has been performed in the framework of the SATURN project with contract no. 100235995 funded by the Europaischer Fonds f\"ur regionale Entwicklung (EFRE) and by the Federal Ministry of Education and Research within the programme "Twenty20 - Partnership for Innovation" under contract 03ZZ0505B - "fast wireless".
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "FilterDesign"
%%% End:

